A Generic Type System for Higher-Order $\Psi$-calculi

The Higher-Order $\Psi$-calculus framework (HO$\Psi$) is a generalisation of many first- and higher-order extensions of the $\pi$-calculus. It was proposed by Parrow et al. who showed that higher-order calculi such as HO$\pi$ and CHOCS can be expressed as HO$\Psi$-calculi. In this paper we present a generic type system for HO$\Psi$-calculi which extends previous work by H\"uttel on a generic type system for first-order $\Psi$-calculi. Our generic type system satisfies the usual property of subject reduction and can be instantiated to yield type systems for variants of HO{\pi}, including the type system for termination due to Demangeon et al. Moreover, we derive a type system for the $\rho$-calculus, a reflective higher-order calculus proposed by Meredith and Radestock. This establishes that our generic type system is richer than its predecessor, as the $\rho$-calculus cannot be encoded in the $\pi$-calculus in a way that satisfies standard criteria of encodability.

==> eptcsdata.tex <==
\providecommand{\firstpage}{43}
\providecommand{\publicationstatus}{V. Castiglioni and C. A. Mezzina (Eds): Combined Workshop on \\ Expressiveness in Concurrency and Structural Operational Semantics 2022 \\ (EXPRESS/SOS 2022).\\
EPTCS 368, 2022, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.368.3}{10.4204/EPTCS.368.3}}
\pdfoutput=1
\usepackage{ifthen}
\providecommand{\eptcs}{{\sl Electronic Proceedings in Theoretical Computer Science}}
\providecommand{\opa}{, Open Publishing Association}
\providecommand{\finishreference}[6]{#1 #2#3, pp. #4--#5, \doi{10.4204/EPTCS.#2.#6}}
\providecommand{\thisvolume}[2][\eptcs]{%
 \ifthenelse{\equal{#2}{2}}{\finishreference{#1}{368}{\opa}{95}{112}{6}}{%
 this volume of #1\opa}}

